CACHEFORGE: LLM-Guided End-to-End Generative Cache Replacement Policy for Performance and Hardware Efficiency

Modern cache replacement designs saturate because they operate within fixed representational structures, hand-crafted and heuristic based feature-engineered predictors, or offline imitation models that cannot generate new decision logic on their own. At the same time, replacement is shaped by the causal interaction of prefetching, thrashing, spatial locality, and access-type behavior, producing an enormous design space that is difficult to traverse manually. Prior approaches typically rely on heuristics, parameter tuning, or imitation of an offline optimal policy, capturing correlations rather than synthesizing new mechanisms. As a result, their performance gains often plateau and they overfit under dynamic workload conditions. CACHEFORGE is the first framework to evolve cache-replacement policies end-to-end by embedding a large language model inside a governed hardware-aware loop. In each iteration, the LLM proposes new C++ replacement logic, the policy is evaluated under a trace-based CRC-2 ChampSim simulator, and the framework enforces feasibility through reward shaping, structural checks, dynamic mutation, temperature scheduling, and cross-policy crossover. This closed-loop generation-evolution loop specifically designed for cache replacement policy enables the discovery of compact policies that satisfy hardware constraints while exploring algorithmic transformations beyond fixed predictor structures. Across SPEC CPU2006, CACHEFORGE outperforms all CRC-2 baselines. It improves the total hit rate by 27.36%, 19.69%, 13.72%, 13.15%, 11.83%, and 5.73% over MPPPB, ReD, Hawk-eye, SHiP++, LIME, and LRU, respectively. On memory-intensive workloads, it increases IPC by 10.15%, 7.89%, 6.34%, 3.64%, 3.12%, and 2.71% over LRU, MPPPB, LIME, ReD, SHiP++, and Hawkeye.

==> Results/IPCvsCHR.tex <==




==> Results/reward.tex <==

% \begin{figure}[!htbp]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%     width=\columnwidth,
%     height=4.5cm,
%     xlabel={Sorted Policies},
%     ylabel={Cache Hit Rate (\%)},
%     xmin=0, xmax=100,
%     ymin=30, ymax=55,
%     tick label style={font=\footnotesize},
%     label style={font=\normalsize},
%     every axis plot/.append style={mark=none,line width=1pt},
%     legend columns=3,
%     legend style={
%         font=\footnotesize,
%         at={(0.5,1)}, % top center
%         anchor=south,
%         draw=none,
%         fill=none,
%     },
% ]

% % --- Weighted Average ---
% \addplot[blue!100!black!40,very thick]
% coordinates {
% (1,50.32)
% (2,50.29)
% (3,50.22)
% (4,50.20)
% (5,50.20)
% (6,50.18)
% (7,50.14)
% (8,50.04)
% (9,49.99)
% (10,49.94)
% (11,49.89)
% (12,49.71)
% (13,49.60)
% (14,49.58)
% (15,49.53)
% (16,49.49)
% (17,49.48)
% (18,49.34)
% (19,49.19)
% (20,49.14)
% (21,49.14)
% (22,49.13)
% (23,49.13)
% (24,49.12)
% (25,49.11)
% (26,49.11)
% (27,49.05)
% (28,49.03)
% (29,49.03)
% (30,48.99)
% (31,48.96)
% (32,48.89)
% (33,48.84)
% (34,48.77)
% (35,48.74)
% (36,48.64)
% (37,48.52)
% (38,48.51)
% (39,48.48)
% (40,48.40)
% (41,48.39)
% (42,48.38)
% (43,48.30)
% (44,48.22)
% (45,48.14)
% (46,48.12)
% (47,47.84)
% (48,47.72)
% (49,47.72)
% (50,47.23)
% (51,47.21)
% (52,47.21)
% (53,47.20)
% (54,47.16)
% (55,47.12)
% (56,47.11)
% (57,47.10)
% (58,47.06)
% (59,46.94)
% (60,46.89)
% (61,46.87)
% (62,46.80)
% (63,46.71)
% (64,46.65)
% (65,46.61)
% (66,46.57)
% (67,46.57)
% (68,46.53)
% (69,46.52)
% (70,46.45)
% (71,46.44)
% (72,46.38)
% (73,46.32)
% (74,46.22)
% (75,45.91)
% (76,45.82)
% (77,45.78)
% (78,45.65)
% (79,45.49)
% (80,45.23)
% (81,45.22)
% (82,45.07)
% (83,44.94)
% (84,44.78)
% (85,44.77)
% (86,44.68)
% (87,44.58)
% (88,44.49)
% (89,44.42)
% (90,43.83)
% (91,43.69)
% (92,43.48)
% (93,43.40)
% (94,42.99)
% (95,42.47)
% (96,42.38)
% (97,40.88)
% (98,40.16)
% (99,36.35)
% };
% \addlegendentry{Weighted Average}

% % --- Hit Rate ---
% \addplot[blue!90!black!70,very thick]
% coordinates {
% (1,49.68)
% (2,49.67)
% (3,49.67)
% (4,49.65)
% (5,49.65)
% (6,49.61)
% (7,49.60)
% (8,48.42)
% (9,48.30)
% (10,48.27)
% (11,48.25)
% (12,48.14)
% (13,48.14)
% (14,48.14)
% (15,48.13)
% (16,48.10)
% (17,48.03)
% (18,47.81)
% (19,47.79)
% (20,47.73)
% (21,47.41)
% (22,47.41)
% (23,47.17)
% (24,47.15)
% (25,47.15)
% (26,47.14)
% (27,47.11)
% (28,47.00)
% (29,46.99)
% (30,46.91)
% (31,46.89)
% (32,46.85)
% (33,46.85)
% (34,46.82)
% (35,46.72)
% (36,46.34)
% (37,46.27)
% (38,46.21)
% (39,46.14)
% (40,46.11)
% (41,45.98)
% (42,45.97)
% (43,45.91)
% (44,45.89)
% (45,45.74)
% (46,45.47)
% (47,45.43)
% (48,45.40)
% (49,45.37)
% (50,45.31)
% (51,45.19)
% (52,45.04)
% (53,44.88)
% (54,44.85)
% (55,44.84)
% (56,44.81)
% (57,44.79)
% (58,44.64)
% (59,44.34)
% (60,43.61)
% (61,43.55)
% (62,43.47)
% (63,42.93)
% (64,42.88)
% (65,40.84)
% (66,38.72)
% (67,38.38)
% (68,36.88)
% };
% \addlegendentry{Hit Rate}

% % --- Average ---
% \addplot[blue!50!black,very thick]
% coordinates {
% (1,49.54)
% (2,49.51)
% (3,49.12)
% (4,48.87)
% (5,48.82)
% (6,48.40)
% (7,48.35)
% (8,48.29)
% (9,48.23)
% (10,48.04)
% (11,47.71)
% (12,47.65)
% (13,47.63)
% (14,47.60)
% (15,47.58)
% (16,47.13)
% (17,46.80)
% (18,46.59)
% (19,46.51)
% (20,46.10)
% (21,46.05)
% (22,46.04)
% (23,45.69)
% (24,45.69)
% (25,45.55)
% (26,45.32)
% (27,44.69)
% (28,44.16)
% (29,44.09)
% (30,43.67)
% (31,43.31)
% (32,43.02)
% (33,42.82)
% (34,42.77)
% (35,42.73)
% (36,42.56)
% (37,42.51)
% (38,42.27)
% (39,42.07)
% (40,42.02)
% (41,41.56)
% (42,41.54)
% (43,41.53)
% (44,41.47)
% (45,41.45)
% (46,41.00)
% (47,40.82)
% (48,40.59)
% (49,40.29)
% (50,40.25)
% (51,40.10)
% (52,40.01)
% (53,40.00)
% (54,39.86)
% (55,39.84)
% (56,39.83)
% (57,39.76)
% (58,39.37)
% (59,39.34)
% (60,39.15)
% (61,38.77)
% (62,38.67)
% (63,38.58)
% (64,38.40)
% (65,38.28)
% (66,38.13)
% (67,37.98)
% (68,37.70)
% (69,37.59)
% (70,37.37)
% (71,37.22)
% (72,36.98)
% (73,36.97)
% (74,36.95)
% (75,36.73)
% (76,36.73)
% (77,36.66)
% (78,36.53)
% (79,36.49)
% (80,36.26)
% (81,35.97)
% (82,35.94)
% (83,35.77)
% (84,35.68)
% (85,35.67)
% (86,35.65)
% (87,35.64)
% (88,35.54)
% (89,35.53)
% (90,32.07)
% };
% \addlegendentry{Average}

% % --- Reference baselines ---
% \addplot[dashed,black!60,thick,domain=0:100]{43.33};
% \node[anchor=west,font=\tiny\bfseries,text=black] at (axis cs:100,43.33){LIME};

% \addplot[dashed,black!60,thick,domain=0:100]{41.69};
% \node[anchor=west,font=\tiny\bfseries,text=black] at (axis cs:100,41.69){LRU};

% \addplot[dashed,black!60,thick,domain=0:100]{37.58};
% \node[anchor=west,font=\tiny\bfseries,text=black] at (axis cs:100,38){Hawkeye};

% \addplot[dashed,black!60,thick,domain=0:100]{37.56};
% \node[anchor=west,font=\tiny\bfseries,text=black] at (axis cs:100,37){SHiP++};

% \addplot[dashed,black!60,thick,domain=0:100]{34.66};
% \node[anchor=west,font=\tiny\bfseries,text=black] at (axis cs:100,34.66){ReD};

% \end{axis}
% \end{tikzpicture}
% \caption{Sorted cache hit rates for policies evolved under Hit Rate, Average, and Weighted Average rewards.} 
% %The weighted formulation achieves the best overall performance, surpassing baseline policies}
% %—LIME (43.3\%), LRU (41.69\%), Hawkeye (37.58\%), SHiP++ (37.56\%), and ReD (34.66\%)—highlighting the impact of reward shaping on policy quality.}
% \label{fig:reward_sorted_onecol}
% \end{figure}


% %\vspace{0.5em}
% \noindent\textbf{Impact of Reward Function} %Design.}
% Each generated policy is scored using a composite reward function that aligns the simulator’s raw statistics with architectural performance goals. 
% We evaluate three formulations: (\textit{i}) a Hit-Rate Reward emphasizing overall cache reuse, (\textit{ii}) an Average Reward combining hit rate and IPC equally, and (\textit{iii}) a Weighted Reward that biases the score toward IPC-critical access types (RFO and load hits). 
% The weighted formulation captures latency-sensitive ownership and demand locality that directly impacts processor throughput. 
% Empirically, this design yields the best performing policies, improving total hit rate by 3–5\% over CRC-2 baselines and demonstrating that reward shaping provides a powerful means of guiding LLM-driven optimization toward high-value microarchitectural trade-offs (see Figure~\ref{fig:reward_sorted_onecol}). %\textcolor{red}{Results go to results. not method.}

% % \vspace{0.5em}
% % \noindent Figure~\ref{fig:reward_sorted_onecol}
% % illustrates the distribution of cache hit rates for policies evolved under different reward functions—raw cache hit rate, average of hit rate and IPC, and a weighted average that biases toward IPC improvement. Policies are sorted in descending order of cache hit rate.
% % %
% % The results show that the weighted reward consistently produces higher-performing policies, with top candidates achieving over 50\% hit rate, surpassing those optimized solely for hit rate or arithmetic average by up to 3–5 percentage points. This demonstrates that reward shaping strongly influences design quality: purely hit-rate-driven objectives favor aggressive insertion but can overfit to short-term reuse, whereas the weighted reward captures both reuse efficiency and latency sensitivity, yielding policies that generalize better across workloads. %Notably, s
% % Several policies optimized under this formulation exceed state-of-the-art baselines such as LIME and Hawkeye, underscoring that the reward function in the feedback loop of \textsc{CacheForge} plays a crucial role in tuning the performance.\textcolor{cyan}{which works better? Previously:} Several policies optimized under this formulation exceed state-of-the-art baselines such as LIME and Hawkeye, underscoring that the \textsc{CacheForge} loop can autonomously discover balanced, cost-aware heuristics without manual tuning.
% % %
% % \textcolor{cyan}{Rewriting Fig 7 analysis}
% % \noindent Figure~\ref{fig:reward_sorted_onecol} shows the distribution of hit rates for policies generated under three reward functions: raw hit rate, an unweighted average of hit rate and IPC, and a weighted formulation that places greater emphasis on IPC. Policies are sorted in descending order of hit rate. 

% % The weighted reward produces the strongest group of policies, with top candidates exceeding 50\% hit rate, approximately 3-5\% on average, higher than those optimized solely for hit rate or the arithmetic average. Hit rate as reward does the second best overall in terms of policies generated. This indicates that reward shaping directly influences the quality of discovered policies,showing that the reward function is a central component of the \textsc{CacheForge} feedback loop. Several policies from this group outperform established baselines such as LIME and Hawkeye, .

% % \textcolor{cyan}{The result from fig 7 (3 reward lines) is counter-intuitive for analysis, because Hit Rate is between the Average and Weighted Average lines. Adding IPC does better in one and somehow worse in the other. How can we explain this?}




% \noindent\textbf{Generalization vs. Overfitting evaluation.} %Additional testing showed that
% To measure generalization capability \textsc{CacheForge} policy autonomously synthesized using only a short 10 M-instruction exploration phase and \textit{five} training workloads, generalizes effectively across all 27 SPEC workloads. On average, it achieves a 3.9\%  %\textcolor{red}{results go to results section not method}
% \textcolor{purple}{What is the relative improvement?} improvement in total hit rate over the best prior policies, consistently outperforming LIME, Hawkeye, SHiP++, and other CRC-2 baselines. Notably, \textsc{CacheForge} attains these gains without hand-crafted heuristics or retraining, demonstrating that LLM-guided policy generation can capture reusable cache-replacement principles that transfer across diverse applications. The uniform uplift observed across both high-reuse (e.g., gamess, perlbench) and memory-intensive workloads (e.g., mcf, milc) indicates that the discovered design balances temporal and spatial reuse behaviors more effectively than prior human-engineered counterparts.
